UIGR: Unified Interactive Garment Retrieval

Interactive garment retrieval (IGR) aims to retrieve a target garment image based on a reference garment image along with user feedback on what to change on the reference garment. Two IGR tasks have been studied extensively: text-guided garment retrieval (TGR) and visually compatible garment retrieval (VCR). The user feedback for the former indicates what semantic attributes to change with the garment category preserved, while the category is the only thing to be changed explicitly for the latter, with an implicit requirement on style preservation. Despite the similarity between these two tasks and the practical need for an efficient system tackling both, they have never been unified and modeled jointly. In this paper, we propose a Unified Interactive Garment Retrieval (UIGR) framework to unify TGR and VCR. To this end, we first contribute a large-scale benchmark suited for both problems. We further propose a strong baseline architecture to integrate TGR and VCR in one model. Extensive experiments suggest that unifying two tasks in one framework is not only more efficient by requiring a single model only, it also leads to better performance. Code and datasets are available at https://github.com/BrandonHanx/CompFashion.

==> images/qualitative_results.tex <==
\begin{figure}[t]
\centering
\subfigure[is \underline{yellow} and with \underline{bead decorations}]{
\includegraphics[width=\linewidth]{figures/tgr_example_1.pdf}
}
\subfigure[is \underline{kimono sleeve} and has \underline{shirt collar}]{
\includegraphics[width=\linewidth]{figures/tgr_example_2.pdf}
}
\subfigure[for this \underline{shirt}, find a visually compatible \underline{pants} with \underline{curved type pocket}]{
\includegraphics[width=\linewidth]{figures/vcr_example_1.pdf}
}
\subfigure[retrieve a \underline{shoe} having a similar style with current \underline{dress}]{
\includegraphics[width=\linewidth]{figures/vcr_example_2.pdf}
}
\caption{Retrieval results of our multi-task framework.
The first two and the last two rows stand for TGR and VCR scenario, respectively.
\textcolor{Dandelion}{Yellow}: reference garment; \textcolor{OrangeRed}{Red}: target garment (ground truth); \textcolor{Cerulean}{Blue}: other retrieved garments.}
\label{fig:qualitative_results}
\vspace*{-2mm}
\end{figure}
